Towards a Step Semantics for Story-Driven Modelling

Graph Transformation (GraTra) provides a formal, declarative means of specifying model transformation. In practice, GraTra rule applications are often programmed via an additional language with which the order of rule applications can be suitably controlled. Story-Driven Modelling (SDM) is a dialect of programmed GraTra, originally developed as part of the Fujaba CASE tool suite. Using an intuitive, UML-inspired visual syntax, SDM provides usual imperative control flow constructs such as sequences, conditionals and loops that are fairly simple, but whose interaction with individual GraTra rules is nonetheless non-trivial. In this paper, we present the first results of our ongoing work towards providing a formal step semantics for SDM, which focuses on the execution of an SDM specification.

==> eptcsdata.tex <==
\providecommand{\firstpage}{42}
\providecommand{\publicationstatus}{Alexander Heu{\ss}ner, Aleks Kissinger, Anton Wijs (Eds.):\\ 2nd Graphs as Models workshop (GaM 2016)\\
EPTCS 231, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.231.4}{10.4204/EPTCS.231.4}}
\pdfoutput=1

